OpenVAM: Open-World Visual Attention Modeling with VLMs

Predicting human gaze is a core capability for applications ranging from web/UI design analysis to robotics and human-computer interaction. Yet, most visual attention modeling methods output only a dense saliency map, which is often insufficient for action: practitioners need to connect attention peaks to discrete elements in the scene (what) and understand the drivers of those peaks in context (why), while remaining robust to domain shift across natural images, commercial content, and UI/web layouts. We, therefore, introduce OpenVAM (Open-world Visual Attention Modeling with VLMs), a unified framework that jointly addresses universality and explainability across heterogeneous domains (natural scenes, commercial imagery, and UI/web layouts) and supervision modalities. OpenVAM adopts a decoupled-but-aligned design: a dedicated dense visual pathway provides stable, spatially precise localization, while an instruction-following vision--language semantic head generates grounded what/why explanations conditioned on the same image and data-type prompts. A three-stage training strategy preserves strong localization priors while progressively introducing language grounding and improving explanation alignment via parameter-efficient adaptation without perturbing the saliency branch. We further propose a scalable pipeline to generate multi-domain saliency-reason annotations for training and systematic evaluation. Experiments across diverse datasets show that OpenVAM improves robustness under domain shift while producing image-grounded explanations that make saliency predictions more interpretable.

==> preamble.tex <==
\RequirePackage[dvipsnames,table]{xcolor}
\usepackage{booktabs}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{rotating}
\usepackage{array}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{placeins}
\usepackage{float}
\usepackage{adjustbox}
\usepackage{subcaption}
\usepackage{xcolor}%
\usepackage[accsupp]{axessibility} % Improves PDF readability for those with disabilities.

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
% Hyperlinked supplement section number (no ``Sec.'' text).
\newcommand{\suppref}[1]{\hyperref[#1]{\ref*{#1}}}
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
\usepackage[most]{tcolorbox}

\newtcolorbox[auto counter, number within=section]{promptbox}[2][]{
colback=pink!10!white,
colframe=red!50!black,
title=#1,
label=#2,
sharp corners,
boxrule=0.5pt,
top=1mm,bottom=1mm,left=2mm,right=2mm
}

==> tables/generalization_table.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Saliency performance on unseen datasets.} OpenVAM generalizes strongly across diverse out-of-distribution benchmarks, with the 7B variant achieving the best overall performance in most cases. Entries marked with ``--'' indicate that the corresponding dataset does not provide fixation annotations required to compute AUC and NSS metrics.}
% \vspace{-0.4em}
\label{tab:saliency_unseen}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{20pt}
\begin{tabular}{c|l|ccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{Saliency Metrics}} \\
\cmidrule(lr){3-7}
& & CC $\uparrow$ & KLD $\downarrow$ & AUC $\uparrow$ & SIM $\uparrow$ & NSS $\uparrow$ \\
\midrule
% ========================= Toronto =========================
\textit{Toronto}~\cite{bruce2007attention} & SUM~\cite{hosseini2025sum}  & 0.767 & 0.558 & 0.875 & 0.642 & 2.170 \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-3B} & \cellcolor[HTML]{DADCFF}0.784 & \cellcolor[HTML]{DADCFF}0.508 & \cellcolor[HTML]{DADCFF}0.882 & \cellcolor[HTML]{DADCFF}0.659 & \cellcolor[HTML]{DADCFF}2.245 \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-7B} & \cellcolor[HTML]{DADCFF}\textbf{0.791} & \cellcolor[HTML]{DADCFF}\textbf{0.499} & \cellcolor[HTML]{DADCFF}\textbf{0.883} & \cellcolor[HTML]{DADCFF}\textbf{0.665} & \cellcolor[HTML]{DADCFF}\textbf{2.254} \\
\midrule
% ========================= TUD Database 1 =========================
\textit{TUD Database 1}~\cite{liu2009studying} & SUM~\cite{hosseini2025sum} & 0.790 & 0.641 & -- & 0.654 & -- \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-3B} & \cellcolor[HTML]{DADCFF}0.720 & \cellcolor[HTML]{DADCFF}0.557 & \cellcolor[HTML]{DADCFF}-- & \cellcolor[HTML]{DADCFF}0.623 & \cellcolor[HTML]{DADCFF}-- \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-7B} & \cellcolor[HTML]{DADCFF}\textbf{0.802} & \cellcolor[HTML]{DADCFF}\textbf{0.555} & \cellcolor[HTML]{DADCFF}-- & \cellcolor[HTML]{DADCFF}\textbf{0.664} & \cellcolor[HTML]{DADCFF}-- \\
\midrule
% ========================= TUD Database 2 =========================
\textit{TUD Database 2}~\cite{alers2010studying} & SUM~\cite{hosseini2025sum} & 0.846 & 0.844 & -- & 0.620 & -- \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-3B} & \cellcolor[HTML]{DADCFF}0.826 & \cellcolor[HTML]{DADCFF}0.804 & \cellcolor[HTML]{DADCFF}-- & \cellcolor[HTML]{DADCFF}0.621 & \cellcolor[HTML]{DADCFF}-- \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-7B} & \cellcolor[HTML]{DADCFF}\textbf{0.854} & \cellcolor[HTML]{DADCFF}\textbf{0.785} & \cellcolor[HTML]{DADCFF}-- & \cellcolor[HTML]{DADCFF}\textbf{0.631} & \cellcolor[HTML]{DADCFF}-- \\
\midrule
% ========================= FIWI =========================
\textit{FIWI}~\cite{shen2014webpage} & SUM~\cite{hosseini2025sum} & 0.678 & 0.542 & 0.818 & 0.613 & 1.428 \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-3B} & \cellcolor[HTML]{DADCFF}0.651 & \cellcolor[HTML]{DADCFF}0.600 & \cellcolor[HTML]{DADCFF}\textbf{0.824} & \cellcolor[HTML]{DADCFF}0.583 & \cellcolor[HTML]{DADCFF}1.378 \\
& \cellcolor[HTML]{DADCFF}\textbf{OpenVAM-7B} & \cellcolor[HTML]{DADCFF}\textbf{0.680} & \cellcolor[HTML]{DADCFF}\textbf{0.538} & \cellcolor[HTML]{DADCFF}0.821 & \cellcolor[HTML]{DADCFF}\textbf{0.626} & \cellcolor[HTML]{DADCFF}\textbf{1.462} \\
\bottomrule
\end{tabular}
}
% \vspace{-0.6em}
\end{table*}

==> tables/qwen_ablation.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Scaling comparison of OpenVAM variants across datasets.}
Each model is built on Qwen-3 VL backbone.}
\vspace{-0.4em}
\label{tab:openvam_scaling_backbone}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|c|c|ccccc|c|ccc|cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} &
\multirow{2}{*}{\textbf{Model}} &
\multirow{2}{*}{\textbf{Backbone}} &
\multirow{2}{*}{\textbf{Params}} &
\multicolumn{5}{c|}{\textbf{Saliency Metrics}} &
\multicolumn{8}{c}{\textbf{Text Generation Metrics}} \\

\cmidrule(lr){5-9}
\cmidrule(lr){10-17}

& & & &
CC $\uparrow$ & KLD $\downarrow$ & AUC $\uparrow$ & SIM $\uparrow$ & NSS $\uparrow$
& JScore $\uparrow$
& R-1 $\uparrow$ & R-2 $\uparrow$ & R-L $\uparrow$
& B-1 $\uparrow$ & B-2 $\uparrow$ & B-3 $\uparrow$ & B-4 $\uparrow$ \\
\midrule

% ===================== U-EYE =====================
\multirow{2}{*}{U-EYE}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
\midrule

% ===================== SalECI =====================
\multirow{2}{*}{SalECI}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
\midrule

% ===================== OSIE =====================
\multirow{2}{*}{OSIE}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
\midrule

% ===================== Salicon =====================
\multirow{2}{*}{Salicon}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
\midrule

% ===================== CAT2000 =====================
\multirow{2}{*}{CAT2000}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
\midrule

% ===================== MIT1003 =====================
\multirow{2}{*}{MIT1003}
& OpenVAM 3 (4B) & Qwen 3 & 4B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\
& OpenVAM 3 (8B) & Qwen 3 & 8B
& -- & -- & -- & -- & --
& --
& -- & -- & --
& -- & -- & -- & -- \\

\bottomrule
\end{tabular}
}
\vspace{-0.6em}
\end{table*}

==> tables/stage_wise_ablation.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Stage-wise ablation of OpenVAM-3B.}
We progressively enable Stage 1 (S1), Stage 2 (S2), and Stage 3 (S3), and also evaluate the alternative strategy where S2 and S3 are jointly trained after S1.}
\vspace{-0.5em}
\label{tab:openvam_stage_ablation_main}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{18pt}
\begin{tabular}{
>{\centering\arraybackslash}p{1.4cm}
>{\centering\arraybackslash}p{0.8cm}
>{\centering\arraybackslash}p{0.8cm}
>{\centering\arraybackslash}p{0.8cm}
|ccccc|c|ccc|cccc
}
\toprule

\multicolumn{4}{c|}{\textbf{Training Stages}}
& \multicolumn{5}{c|}{\textbf{Saliency}}
& \multicolumn{1}{c|}{\textbf{VLM Judge} $\uparrow$}
& \multicolumn{3}{c|}{\textbf{ROUGE} $\uparrow$}
& \multicolumn{4}{c}{\textbf{BLEU} $\uparrow$} \\

\midrule

Dataset & S1 & S2 & S3
& CC $\uparrow$ & KLD $\downarrow$ & AUC $\uparrow$ & SIM $\uparrow$ & NSS $\uparrow$
& JScore
& R-1 & R-2 & R-L
& B-1 & B-2 & B-3 & B-4 \\

\midrule

% ================= U-EYE =================
\multirow{4}{*}{{U-EYE}~\cite{jiang2023ueyes}}
& \cmark & \xmark & \xmark
& 0.728 & 0.550 & 0.846 & 0.622 & 1.704
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& 0.730 & 0.559 & 0.845 & 0.620 & 1.714
& 0.441 & 0.388 & 0.083 & 0.181
& 0.271 & 0.113 & 0.050 & 0.026 \\

& \cmark & \cmark & \xmark
& 0.735 & 0.543 & 0.847 & 0.630 & 1.721
& 0.434 & 0.252 & 0.034 & 0.133
& 0.148 & 0.050 & 0.019 & 0.009 \\

& \cmark & \cmark & \cmark
& 0.734 & 0.542 & 0.847 & 0.639 & 1.720
& 0.603 & 0.429 & 0.108 & 0.196
& 0.330 & 0.156 & 0.077 & 0.040 \\

\midrule

% ================= SalECI =================
\multirow{4}{*}{SalECI~\cite{jiang2022does}}
& \cmark & \xmark & \xmark
& 0.788 & 0.466 & 0.898 & 0.675 & 2.031
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& 0.790 & 0.465 & 0.889 & 0.678 & 2.032
& 0.382 & 0.395 & 0.090 & 0.186
& 0.244 & 0.109 & 0.052 & 0.027 \\

& \cmark & \cmark & \xmark
& 0.792 & 0.464 & 0.899 & 0.680 & 2.035
& 0.376 & 0.244 & 0.023 & 0.136
& 0.159 & 0.046 & 0.020 & 0.010 \\

& \cmark & \cmark & \cmark
& 0.795 & 0.462 & 0.899 & 0.680 & 2.026
& 0.692 & 0.478 & 0.130 & 0.220
& 0.369 & 0.184 & 0.096 & 0.050 \\

\midrule

% ================= OSIE =================
\multirow{4}{*}{OSIE~\cite{xu2014predicting}}
& \cmark & \xmark & \xmark
& 0.912 & 0.229 & 0.935 & 0.777 & 3.903
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& -- & -- & -- & -- & --
& -- & -- & -- & --
& -- & -- & -- & -- \\

& \cmark & \cmark & \xmark
& 0.922 & 0.232 & 0.934 & 0.783 & 3.743
& 0.497 & 0.270 & 0.027 & 0.146
& 0.200 & 0.060 & 0.025 & 0.012 \\

& \cmark & \cmark & \cmark
& 0.928 & 0.214 & 0.935 & 0.793 & 3.841
& 0.661 & 0.472 & 0.123 & 0.220
& 0.364 & 0.178 & 0.089 & 0.047 \\

\midrule

% ================= Salicon =================
\multirow{4}{*}{Salicon~\cite{jiang2015salicon}}
& \cmark & \xmark & \xmark
& 0.902 & 0.186 & 0.875 & 0.799 & 1.985
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& -- & -- & -- & -- & --
& -- & -- & -- & --
& -- & -- & -- & -- \\

& \cmark & \cmark & \xmark
& 0.922 & 0.232 & 0.934 & 0.783 & 3.743
& 0.497 & 0.270 & 0.027 & 0.146
& 0.200 & 0.060 & 0.025 & 0.012 \\

& \cmark & \cmark & \cmark
& 0.911 & 0.184 & 0.876 & 0.805 & 1.989
& 0.677 & 0.424 & 0.157 & 0.211
& 0.342 & 0.163 & 0.097 & 0.055 \\

\midrule

% ================= CAT2000 =================
\multirow{4}{*}{CAT2000~\cite{borji2015cat2000}}
& \cmark & \xmark & \xmark
& 0.884 & 0.262 & 0.888 & 0.754 & 2.438
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& -- & -- & -- & -- & --
& -- & -- & -- & --
& -- & -- & -- & -- \\

& \cmark & \cmark & \xmark
& 0.892 & 0.256 & 0.888 & 0.760 & 2.450
& 0.552 & 0.230 & 0.017 & 0.136
& 0.169 & 0.045 & 0.019 & 0.010 \\

& \cmark & \cmark & \cmark
& 0.891 & 0.258 & 0.889 & 0.759 & 2.452
& 0.663 & 0.442 & 0.111 & 0.217
& 0.333 & 0.162 & 0.081 & 0.043 \\

\midrule

% ================= MIT1003 =================
\multirow{4}{*}{MIT1003~\cite{judd2009learning}}
& \cmark & \xmark & \xmark
& 0.817 & 0.483 & 0.922 & 0.656 & 3.050
& -- & -- & -- & -- & -- & -- & -- & -- \\

& \cmark & \multicolumn{2}{c|}{joint}
& -- & -- & -- & -- & --
& -- & -- & -- & --
& -- & -- & -- & -- \\

& \cmark & \cmark & \xmark
& 0.820 & 0.483 & 0.921 & 0.661 & 3.020
& 0.453 & 0.249 & 0.022 & 0.142
& 0.184 & 0.053 & 0.023 & 0.012 \\

& \cmark & \cmark & \cmark
& 0.829 & 0.463 & 0.923 & 0.671 & 3.081
& 0.659 & 0.447 & 0.111 & 0.217
& 0.335 & 0.161 & 0.080 & 0.043 \\

\bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\end{table*}



% \begin{table*}[t]
% \centering
% \caption{\textbf{Stage-wise ablation of OpenVAM-3B.}
% We progressively enable Stage 1 (S1), Stage 2 (S2), and Stage 3 (S3).}
% \vspace{-0.5em}
% \label{tab:openvam_stage_ablation_main}
% \resizebox{\textwidth}{!}{
% \setlength{\tabcolsep}{8pt}
% \begin{tabular}{
% >{\centering\arraybackslash}p{1.4cm}
% >{\centering\arraybackslash}p{0.8cm}
% >{\centering\arraybackslash}p{0.8cm}
% >{\centering\arraybackslash}p{0.8cm}
% |ccccc|c|ccc|cccc
% }
% \toprule

% \multicolumn{4}{c|}{\textbf{Training Stages}}
% & \multicolumn{5}{c|}{\textbf{Saliency}}
% & \multicolumn{1}{c|}{\textbf{VLM Judge} $\uparrow$}
% & \multicolumn{3}{c|}{\textbf{ROUGE} $\uparrow$}
% & \multicolumn{4}{c}{\textbf{BLEU} $\uparrow$} \\

% \midrule

% Dataset & S1 & S2 & S3
% & CC $\uparrow$ & KLD $\downarrow$ & AUC $\uparrow$ & SIM $\uparrow$ & NSS $\uparrow$
% & JScore
% & R-1 & R-2 & R-L
% & B-1 & B-2 & B-3 & B-4 \\

% \midrule

% % ================= U-EYE =================
% \multirow{3}{*}{{U-EYE}~\cite{jiang2023ueyes}}
% & \cmark & \xmark & \xmark & 0.728 & 0.550 & 0.846 & 0.622 & 1.704 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.735 & 0.543 & 0.847 & 0.630 & 1.721
% & 0.434 & 0.252 & 0.034 & 0.133
% & 0.148 & 0.050 & 0.019 & 0.009 \\
% & \cmark & \cmark & \cmark & 0.734 & 0.542 & 0.847 & 0.639 & 1.720
% & 0.603 & 0.429 & 0.108 & 0.196
% & 0.330 & 0.156 & 0.077 & 0.040 \\
% \midrule

% % ================= SalECI =================
% \multirow{3}{*}{SalECI~\cite{jiang2022does}}
% & \cmark & \xmark & \xmark & 0.788 & 0.466 & 0.898 & 0.675 & 2.031 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.792 & 0.464 & 0.899 & 0.680 & 2.035
% & 0.376 & 0.244 & 0.023 & 0.136
% & 0.159 & 0.046 & 0.020 & 0.010 \\
% & \cmark & \cmark & \cmark & 0.795 & 0.462 & 0.899 & 0.680 & 2.026
% & 0.692 & 0.478 & 0.130 & 0.220
% & 0.369 & 0.184 & 0.096 & 0.050 \\
% \midrule

% % ================= OSIE =================
% \multirow{3}{*}{OSIE~\cite{xu2014predicting}}
% & \cmark & \xmark & \xmark & 0.912 & 0.229 & 0.935 & 0.777 & 3.903 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.922 & 0.232 & 0.934 & 0.783 & 3.743
% & 0.497 & 0.270 & 0.027 & 0.146
% & 0.200 & 0.060 & 0.025 & 0.012 \\
% & \cmark & \cmark & \cmark & 0.928 & 0.214 & 0.935 & 0.793 & 3.841
% & 0.661 & 0.472 & 0.123 & 0.220
% & 0.364 & 0.178 & 0.089 & 0.047 \\
% \midrule

% % ================= Salicon =================
% \multirow{3}{*}{Salicon~\cite{jiang2015salicon}}
% & \cmark & \xmark & \xmark & 0.902 & 0.186 & 0.875 & 0.799 & 1.985 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.922 & 0.232 & 0.934 & 0.783 & 3.743
% & 0.497 & 0.270 & 0.027 & 0.146
% & 0.200 & 0.060 & 0.025 & 0.012 \\
% & \cmark & \cmark & \cmark & 0.911 & 0.184 & 0.876 & 0.805 & 1.989
% & 0.677 & 0.424 & 0.157 & 0.211
% & 0.342 & 0.163 & 0.097 & 0.055 \\
% \midrule

% % ================= CAT2000 =================
% \multirow{3}{*}{CAT2000~\cite{borji2015cat2000}}
% & \cmark & \xmark & \xmark & 0.884 & 0.262 & 0.888 & 0.754 & 2.438 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.892 & 0.256 & 0.888 & 0.760 & 2.450
% & 0.552 & 0.230 & 0.017 & 0.136
% & 0.169 & 0.045 & 0.019 & 0.010 \\
% & \cmark & \cmark & \cmark & 0.891 & 0.258 & 0.889 & 0.759 & 2.452
% & 0.663 & 0.442 & 0.111 & 0.217
% & 0.333 & 0.162 & 0.081 & 0.043 \\
% \midrule

% % ================= MIT1003 =================
% \multirow{3}{*}{MIT1003~\cite{judd2009learning}}
% & \cmark & \xmark & \xmark & 0.817 & 0.483 & 0.922 & 0.656 & 3.050 & -- & -- & -- & -- & -- & -- & -- & -- \\
% & \cmark & \cmark & \xmark & 0.820 & 0.483 & 0.921 & 0.661 & 3.020
% & 0.453 & 0.249 & 0.022 & 0.142
% & 0.184 & 0.053 & 0.023 & 0.012 \\
% & \cmark & \cmark & \cmark & 0.829 & 0.463 & 0.923 & 0.671 & 3.081
% & 0.659 & 0.447 & 0.111 & 0.217
% & 0.335 & 0.161 & 0.080 & 0.043 \\

% \bottomrule
% \end{tabular}
% }
% % \vspace{-1.5em}
% \end{table*}
